PolypConnect: Image inpainting for generating realistic gastrointestinal tract images with polyps

Early identification of a polyp in the lower gastrointestinal (GI) tract can lead to prevention of life-threatening colorectal cancer. Developing computer-aided diagnosis (CAD) systems to detect polyps can improve detection accuracy and efficiency and save the time of the domain experts called endoscopists. Lack of annotated data is a common challenge when building CAD systems. Generating synthetic medical data is an active research area to overcome the problem of having relatively few true positive cases in the medical domain. To be able to efficiently train machine learning (ML) models, which are the core of CAD systems, a considerable amount of data should be used. In this respect, we propose the PolypConnect pipeline, which can convert non-polyp images into polyp images to increase the size of training datasets for training. We present the whole pipeline with quantitative and qualitative evaluations involving endoscopists. The polyp segmentation model trained using synthetic data, and real data shows a 5.1% improvement of mean intersection over union (mIOU), compared to the model trained only using real data. The codes of all the experiments are available on GitHub to reproduce the results.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)
SAMPLEBIBLATEXFILES=$(patsubst %,samples/%,$(BIBLATEXFILES))

all:  ${PDF} ALLSAMPLES

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > samples/abbrev.bib 


samples/%.bbx: %.bbx
samples/%.cbx: %.cbx
samples/%.dbx: %.dbx
samples/%.lbx: %.lbx

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-sigconf-biblatex.pdf: samples/sample-sigconf-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-acmsmall-biblatex.pdf: samples/sample-acmsmall-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut \
	samples/*.run.xml samples/*.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

Version 1.84   Support for BibLaTeX rewritten (thanks to
	       Roberto Di Cosmo and Kartik Singhal)
	       Corrected German translation (thanks to Dirk Beyer)
	       New journals

Version 1.83   Support for multilanguage papers
	       ISSN changes for some journals

Version 1.82   Bug fixes.
	       New command \anon for anonymization of short strings.
	       Documentation update.

Version 1.81   Bug fixes
	       New bib field distinctURL to print URL even if doi is present.
	       Reworded samples

Version 1.80   New journals: DLT, FAC

Version 1.79   Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

Version 1.78   Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.77   Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.76   Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.75   \country is now obligatory for addresses.
	       Added \AtBeginMaketitle

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.63a   Moved TQUANT to TQC

Version 1.63	New journals: TQUANT, FACMP

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.52    Another rewording of licenses

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.49    New jorunal:  DTRAP

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.47    New journal: THRI

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.43    Bug fixes

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.41    Rearranged bib files
                Added new badges

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.39    Added \authornotemark commmand

Version 1.38    Increase default font size for SIGPLAN

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

Version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

Version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

Version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

Version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

Version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

Version 1.28    Bug fixes: natbib=false now behaves correctly.

Version 1.27    Bug fixes

Version 1.26    Bug fixes

Version 1.25    Updated PACMPL journal option.

Version 1.24    Added IMWUT journal option.

Version 1.23    Added PACM PL journal option.

Version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

Version 1.21    Bibliography changes: added arXiv, some cleanup

Version 1.20    Bug fixes, documentation updates

Version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

Version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.


Version 1.17    Formatting changes for margins and lists.  Bug fixes.

Version 1.16    Formatting changes for headers and footers.

Version 1.15    New structured affiliation command.
                New commands for acknowledgements.

Version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

Version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

Version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

Version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

Version 1.10    Bug fixes

Version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

Version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes


==> figure_tex/edge_connect_results_v2.tex <==
\begin{figure}
    \centering
    \setlength{\tabcolsep}{1pt}
    \newcommand{\imgwidth}{0.15\linewidth}
    \begin{tabular}{p{0.4cm}ccccccc}
    
        
        \multirow{-8}{*}{(a)} &
        \includegraphics[width=\imgwidth]{images/original_polyps/cju183od81ff608017ekzif89.jpg} &
        \includegraphics[width=\imgwidth]{images/original_polyps/cju31rb7vb6110801p9rhacuw.jpg} &
        \includegraphics[width=\imgwidth]{images/original_polyps/cju42g865lorv07552ytz6xxa.jpg} &
        \includegraphics[width=\imgwidth]{images/original_polyps/cju42wamblrqn098798r2yyok.jpg} &
        \includegraphics[width=\imgwidth]{images/original_polyps/cju6vvxsev9y30987kespucdg.jpg} &
        \includegraphics[width=\imgwidth]{images/original_polyps/cju7bgnvb1sf808717qa799ir.jpg}
        \\
        
        \multirow{-8}{*}{(b)} &
        \includegraphics[width=\imgwidth]{images/EDGECONNECT/FINETUNED/ori_mask/0d07d365-d6e1-4dca-99b7-c57b457f37b1_cju183od81ff608017ekzif89.jpg} &
        \includegraphics[width=\imgwidth]{images/EDGECONNECT/FINETUNED/ori_mask/4536139f-65ac-45a1-ad1c-a7d160fb2509_cju31rb7vb6110801p9rhacuw.jpg} &
        \includegraphics[width=\imgwidth]{images/EDGECONNECT/FINETUNED/ori_mask/6ea3e705-c59d-41f3-95aa-d7e1051ea245_cju42g865lorv07552ytz6xxa.jpg} &
        \includegraphics[width=\imgwidth]{images/EDGECONNECT/FINETUNED/ori_mask/72b19e66-278e-487c-8748-4e56aa44049e_cju42wamblrqn098798r2yyok.jpg} &
        \includegraphics[width=\imgwidth]{images/EDGECONNECT/FINETUNED/ori_mask/a39b14bc-dfb5-46ab-8246-606932986b7a_cju6vvxsev9y30987kespucdg.jpg} &
        \includegraphics[width=\imgwidth]{images/EDGECONNECT/FINETUNED/ori_mask/bb15dcc7-2ac8-4e1a-be61-53fa10ea60a6_cju7bgnvb1sf808717qa799ir.jpg}
        
        \\
        
        
        
        
        \multirow{-8}{*}{(c)} &
        \includegraphics[width=\imgwidth]{images/EDGECONNECT/FINETUNED/ori_mask/0d07d365-d6e1-4dca-99b7-c57b457f37b1.jpg} & 
        \includegraphics[width=\imgwidth]{images/EDGECONNECT/FINETUNED/ori_mask/4536139f-65ac-45a1-ad1c-a7d160fb2509.jpg} &
        \includegraphics[width=\imgwidth]{images/EDGECONNECT/FINETUNED/ori_mask/6ea3e705-c59d-41f3-95aa-d7e1051ea245.jpg} &
        \includegraphics[width=\imgwidth]{images/EDGECONNECT/FINETUNED/ori_mask/72b19e66-278e-487c-8748-4e56aa44049e.jpg} &
        \includegraphics[width=\imgwidth]{images/EDGECONNECT/FINETUNED/ori_mask/a39b14bc-dfb5-46ab-8246-606932986b7a.jpg} &
        \includegraphics[width=\imgwidth]{images/EDGECONNECT/FINETUNED/ori_mask/bb15dcc7-2ac8-4e1a-be61-53fa10ea60a6.jpg}
        
        \\
        
        \multirow{-8}{*}{(d)} &
        \includegraphics[width=\imgwidth]{images/EDGECONNECT/FINETUNED/without_edges/6_image_edge_0d07d365-d6e1-4dca-99b7-c57b457f37b1.jpg} &
        \includegraphics[width=\imgwidth]{images/EDGECONNECT/FINETUNED/without_edges/48_image_edge_4536139f-65ac-45a1-ad1c-a7d160fb2509.jpg} &
        \includegraphics[width=\imgwidth]{images/EDGECONNECT/FINETUNED/without_edges/77_image_edge_6ea3e705-c59d-41f3-95aa-d7e1051ea245.jpg} &
        \includegraphics[width=\imgwidth]{images/EDGECONNECT/FINETUNED/without_edges/80_image_edge_72b19e66-278e-487c-8748-4e56aa44049e.jpg} &
        \includegraphics[width=\imgwidth]{images/EDGECONNECT/FINETUNED/without_edges/114_image_edge_a39b14bc-dfb5-46ab-8246-606932986b7a.jpg} &
        \includegraphics[width=\imgwidth]{images/EDGECONNECT/FINETUNED/without_edges/132_image_edge_bb15dcc7-2ac8-4e1a-be61-53fa10ea60a6.jpg} &
        
        \\
        
        \multirow{-8}{*}{(e)} &
        \includegraphics[width=\imgwidth]{images/EDGECONNECT/FINETUNED/with_edges/6_polyp_edge_cju183od81ff608017ekzif89.jpg} &
        \includegraphics[width=\imgwidth]{images/EDGECONNECT/FINETUNED/with_edges/48_polyp_edge_cju31rb7vb6110801p9rhacuw.jpg} &
        \includegraphics[width=\imgwidth]{images/EDGECONNECT/FINETUNED/with_edges/77_polyp_edge_cju42g865lorv07552ytz6xxa.jpg} &
        \includegraphics[width=\imgwidth]{images/EDGECONNECT/FINETUNED/with_edges/80_polyp_edge_cju42wamblrqn098798r2yyok.jpg} &
        \includegraphics[width=\imgwidth]{images/EDGECONNECT/FINETUNED/with_edges/114_polyp_edge_cju6vvxsev9y30987kespucdg.jpg} &
        \includegraphics[width=\imgwidth]{images/EDGECONNECT/FINETUNED/with_edges/132_polyp_edge_cju7bgnvb1sf808717qa799ir.jpg} 
        
        \\
        
        
        \multirow{-8}{*}{(f)} &
         \includegraphics[width=\imgwidth]{images/EDGECONNECT/FINETUNED/with_edges/6_merged_edges_0d07d365-d6e1-4dca-99b7-c57b457f37b1.jpg} &
        \includegraphics[width=\imgwidth]{images/EDGECONNECT/FINETUNED/with_edges/48_merged_edges_4536139f-65ac-45a1-ad1c-a7d160fb2509.jpg} &
        \includegraphics[width=\imgwidth]{images/EDGECONNECT/FINETUNED/with_edges/77_merged_edges_6ea3e705-c59d-41f3-95aa-d7e1051ea245.jpg} &
        \includegraphics[width=\imgwidth]{images/EDGECONNECT/FINETUNED/with_edges/80_merged_edges_72b19e66-278e-487c-8748-4e56aa44049e.jpg} &
        \includegraphics[width=\imgwidth]{images/EDGECONNECT/FINETUNED/with_edges/114_merged_edges_a39b14bc-dfb5-46ab-8246-606932986b7a.jpg} &
        \includegraphics[width=\imgwidth]{images/EDGECONNECT/FINETUNED/with_edges/132_merged_edges_bb15dcc7-2ac8-4e1a-be61-53fa10ea60a6.jpg} 
        
        \\
        
        \multirow{-8}{*}{(g)} &
        \includegraphics[width=\imgwidth]{images/EDGECONNECT/FINETUNED/with_edges/0d07d365-d6e1-4dca-99b7-c57b457f37b1_with_edge.jpg} &
        \includegraphics[width=\imgwidth]{images/EDGECONNECT/FINETUNED/with_edges/4536139f-65ac-45a1-ad1c-a7d160fb2509_with_edge.jpg} &
        \includegraphics[width=\imgwidth]{images/EDGECONNECT/FINETUNED/with_edges/6ea3e705-c59d-41f3-95aa-d7e1051ea245_with_edge.jpg} &
        \includegraphics[width=\imgwidth]{images/EDGECONNECT/FINETUNED/with_edges/72b19e66-278e-487c-8748-4e56aa44049e_with_edge.jpg} &
        \includegraphics[width=\imgwidth]{images/EDGECONNECT/FINETUNED/with_edges/a39b14bc-dfb5-46ab-8246-606932986b7a_with_edge.jpg} &
        \includegraphics[width=\imgwidth]{images/EDGECONNECT/FINETUNED/with_edges/bb15dcc7-2ac8-4e1a-be61-53fa10ea60a6_with_edge.jpg}
         \\
         
         \multirow{-8}{*}{(h)} &
         \includegraphics[width=\imgwidth]{images/AOTGAN/FINETUNED/0d07d365-d6e1-4dca-99b7-c57b457f37b1.png} &
        \includegraphics[width=\imgwidth]{images/AOTGAN/FINETUNED/4536139f-65ac-45a1-ad1c-a7d160fb2509.png} &
        \includegraphics[width=\imgwidth]{images/AOTGAN/FINETUNED/6ea3e705-c59d-41f3-95aa-d7e1051ea245.png} &
        \includegraphics[width=\imgwidth]{images/AOTGAN/FINETUNED/72b19e66-278e-487c-8748-4e56aa44049e.png} &
        \includegraphics[width=\imgwidth]{images/AOTGAN/FINETUNED/a39b14bc-dfb5-46ab-8246-606932986b7a.png} &
        \includegraphics[width=\imgwidth]{images/AOTGAN/FINETUNED/bb15dcc7-2ac8-4e1a-be61-53fa10ea60a6.png}
         
         
        
    \end{tabular}
    
    \caption{Sample data used and generated in the different steps of PolypConnect pipeline. \textbf{(a)} - real polyp images, \textbf{(b)} - manually annotated polyp masks, \textbf{(c)} - randomly selected colon images used as input to the final step of PolypConnect, \textbf{(d)} - extracted edge images of row \textbf{c}. \textbf{(e)} - extracted edge images of polyp regions of row \textbf{a} using the masks of row \textbf{b}. \textbf{(f)} - combined edge images of row \textbf{d} and \textbf{f}. \textbf{(g)} - generated polyp on the images of row \textbf{c} using EdgeConnect. \textbf{(h)} - generated samples from AOTGAN.}
    \label{fig:gen_samples}
    \vspace{-20pt}
\end{figure}

